CDSD: Chinese Dysarthria Speech Database

Dysarthric speech poses significant challenges for individuals with dysarthria, impacting their ability to communicate socially. Despite the widespread use of Automatic Speech Recognition (ASR), accurately recognizing dysarthric speech remains a formidable task, largely due to the limited availability of dysarthric speech data. To address this gap, we developed the Chinese Dysarthria Speech Database (CDSD), the most extensive collection of Chinese dysarthria data to date, featuring 133 hours of recordings from 44 speakers. Our benchmarks reveal a best Character Error Rate (CER) of 16.4\%. Compared to the CER of 20.45\% from our additional human experiments, Dysarthric Speech Recognition (DSR) demonstrates its potential in significant improvement of communication for individuals with dysarthria. The CDSD database will be made publicly available at http://melab.psych.ac.cn/CDSD.html.

==> backup_name.tex <==
% the order of authors here must exactly match the order entered into the paper submission system
% note that the COMPLETE list of authors MUST be entered into the paper submission system at the outset, including when submitting your manuscript for double-blind review
\name[affiliation={1,2}]{Yan}{Wang}
\name[affiliation={1,2}]{Mengyi}{Sun}
\name[affiliation={3}]{Xinchen}{Kang}
\name[affiliation={4}]{Pengfei}{Guo}
\name[affiliation={5}]{Ming}{Gao}
\name[affiliation={1,2}]{Su-Jing}{Wang}
%The maximum number of authors in the author list is 20. If the number of contributing authors is more than this, they should be listed in a footnote or the acknowledgement section.

% if you have too many addresses to fit within the available space, try removing the "\\" newlines
\address{
  $^1$CAS Key Laboratory of Behavioral Science, Institute of Psychology, China\\
  $^2$Department of Psychology, University of the Chinese Academy of Sciences, China\\
  $^3$Beijing Key Laboratory of Information Service Engineering, Beijing Union University, China\\
  $^4$School of Computer Science, Jiangsu University of Science and Technology, China\\
  $^5$University of Science and Technology of China, China}
  
\email{first@university.edu, second@companyA.com, third@companyB.ai}

